Give Me the Facts! A Survey on Factual Knowledge Probing in Pre-trained Language Models

Pre-trained Language Models (PLMs) are trained on vast unlabeled data, rich in world knowledge. This fact has sparked the interest of the community in quantifying the amount of factual knowledge present in PLMs, as this explains their performance on downstream tasks, and potentially justifies their use as knowledge bases. In this work, we survey methods and datasets that are used to probe PLMs for factual knowledge. Our contributions are: (1) We propose a categorization scheme for factual probing methods that is based on how their inputs, outputs and the probed PLMs are adapted; (2) We provide an overview of the datasets used for factual probing; (3) We synthesize insights about knowledge retention and prompt optimization in PLMs, analyze obstacles to adopting PLMs as knowledge bases and outline directions for future work.

==> src/08_conclusion_draft.tex <==




%In this survey, we introduced a categorization for probing methods that depends on how the probing inputs, the probed PLMs and their outputs are adapted to extract more facts from PLMs. Furthermore, we provided an overview of datasets that are used for factual knowledge probing and categorized these datasets under three classes depending on their usage. Additionally, we summarized insights about knowledge retention in PLMs and prompts optimization, and went over obstacles and recent countermeasures to using PLMs as knowledge bases.

%%%%
%PLMs can be probed for factual knowledge in various ways. Besides having fair estimates about factual knowledge, it is essential to have grounded conclusions based on these estimates. PLMs as KBs is a promising direction, but faces significant challenges. Promising directions for future work are addressing these challenges and exploring the potentials of recently published large PLMs, e.g.,~\cite{touvron-etal-2023-llama, penedo-etal-2023-falcon}.

%%%% 
%Making further progress in addressing these challenges and exploring the potentials of more knowledgeable PLMs are possible directions for future work.

%suggestion:
%\CS{Promising directions for future work are addressing these challenges and exploring the potential of recently published LLMs, such as XXX\cite{}.}


\begin{comment}

Querying PLMs for knowledge is desireable for many reasons (e.g., queries in natural language, no labeling effort), but they come with serious limitations as well. Improving the consistency of PLMs, and making them interpretable and updateable are essential future directions for the use of PLMs as KBs. 

Although the knowledge present in PLMs can be scaled by adding more parameters and training on larger corpora, we believe it is crucial to focus PLMs more sustainable by creating smaller and more specialized PLMs, that are accessible for more researchers. 

Another future direction is generating labeled training data where knowledgeable PLMs could play a crucial role, as more knowledgeable PLMs would translate into more diverse data.  

\end{comment}


==> src/08_future_work.tex <==
% Future work
Promising directions for future work include addressing the challenges to adopting PLMs as KBs, investigating factual knowledge in the recently published large PLMs, e.g.,~\cite{openai-2023-gpt4, penedo-etal-2023-falcon, touvron-etal-2023-llama}, and developing comprehensive probing benchmarks that correspond to the capacity of these models.

==> src/prelimnaries_draft.tex <==
%Probing for factual knowledge involves having a PLM, which we are interested in knowing how much factual knowledge it encodes, and a dataset to evaluate that. The dataset contains inputs that identify the fact we are looking for, in order to extract it from the PLM (e.g., ``Dante was born in \texttt{[MASK]}'', and ground truth answers that help evaluate if the retrieved answers are indeed correct (e.g., Florence). The data is also often described in terms of relations (e.g., ``place-of-birth''), subjects (e.g., ``Dante'') and objects (e.g., ``Florence''). A template is created for each relation (e.g., `[X] was born in \texttt{[MASK]}''), that is then filled with subject entities. The inputs could also be formulated as questions (e.g., ``Where was Dante born?'').  

%We only consider works that target the factual knowledge encoded in PLMs, i.e., works that do intrinsic evaluations~\cite{kalyan-etal-2021-ammus}, and exclude works that do extrinsic evaluations on downstream tasks. 


%We also exclude PLMs that are not pre-trained on unlabeled text corpora. 

